IBM Functional Genomics Platform, A Cloud-Based Platform for Studying Microbial Life at Scale

The rapid growth in biological sequence data is revolutionizing our understanding of genotypic diversity and challenging conventional approaches to informatics. With the increasing availability of genomic data, traditional bioinformatic tools require substantial computational time and the creation of ever-larger indices each time a researcher seeks to gain insight from the data. To address these challenges, we pre-computed important relationships between biological entities spanning the Central Dogma of Molecular Biology and captured this information in a relational database. The database can be queried across hundreds of millions of entities and returns results in a fraction of the time required by traditional methods. In this paper, we describe \textit{IBM Functional Genomics Platform} (formerly known as OMXWare), a comprehensive database relating genotype to phenotype for bacterial life. Continually updated, IBM Functional Genomics Platform today contains data derived from 200,000 curated, self-consistently assembled genomes. The database stores functional data for over 68 million genes, 52 million proteins, and 239 million domains with associated biological activity annotations from Gene Ontology, KEGG, MetaCyc, and Reactome. IBM Functional Genomics Platform maps all of the many-to-many connections between each biological entity including the originating genome, gene, protein, and protein domain. Various microbial studies, from infectious disease to environmental health, can benefit from the rich data and connections. We describe the data selection, the pipeline to create and update the IBM Functional Genomics Platform, and the developer tools (Python SDK and REST APIs) which allow researchers to efficiently study microbial life at scale.

==> section_discovery.tex <==
In this section, we will highlight the discovery potential when using the OMXWare database through an example of finding features relevant to the virulence phenotype. We leverage the fact than in bacterial genomes, genes that are often expressed together often exist near each other in gene-clusters on the chromosome. We built an application on top of OMXWare to expand the scope of feature discovery beyond an initial gene set. For example, beginning with a set of input domains, we find all gene features with the known domain architecture and then perform a relative gene position analysis to find additional neighboring proteins that provide high sensitivity and specificity.

We begin by starting with a list of 34 unique genes by name known to be relevant to a particular virulence phenotype. This gene set was introduced by a domain expert, which resulted in 146 domain codes using the OMXWare system. We then found the common functional domain codes and architectures (combinations of IPR codes) across the input genes. This set of domain combinations became our initial set for analysis. We then found all proteins within OMXWare that contain any of these domain combinations. We called this protein set "pivot proteins", as they are the proteins used as reference points to find adjacent proteins. We then found all genomes containing one or more pivot proteins. In order to be sensitive and specific, we ignored any genome that does not contain more than 10 original domains, creating an in-group and out-group of genomes. This is to avoid including genomes that may not display the virulence phenotype in the analysis. For all pivot proteins, we calculated the log-scale ratio of number of times it appears in an in-group genome to number of times it appears in an out-group genome. We then select only those pivot proteins that are at a log-scale ratio of 0 or higher to find the two adjacent (neighbor) proteins on its genome. We find the neighbor proteins using the Prokka index $i$ of the pivot protein on a given genome and return the two proteins at location $i+1$ and $i-1$ on the same genome. If the neighbor protein was also one of the original pivot proteins, we call that a co-pivot protein. If the neighbor protein was not included in the original set, this is a discovered protein. Using this discovered protein set, we can augment the known proteins that contribute to the particular virulence phenotype. Using our methods, we found 114 uniquely named pivot proteins and 66 uniquely named discovered proteins, across genomes in the database.

Thus, we can see that the structure of the OMXWare database is crucial to this analysis, as we traverse from domains to proteins to genomes to identifying adjacent proteins. Without a relational database to facilitate these connections, such analysis would not be possible on a large scale. This application is contributed back to the community and deployed as a micro-service within OMXWare to allow researchers to discover features relevant to any phenotype of interest. This application can be accessed through the OMXWare Applications page. 



==> section_editing_notes.tex <==
This section will be removed later. It serves as a place for us to capture notes or TODOs as we work on the manuscript.

\subsection{Potential journals}
\textcolor{red}{Any others?}
\begin{itemize}
    \item submit as bioRxiv pre-print early to have a DOI for citation and garner support on road to publication
    \item IEEE/ACM Comp Bio and Bioinformatics (editorial approval in progress)
    \item BioData Mining (focus on scale https://biodatamining.biomedcentral.com/)
    \item PLOS Computational Bio
    \item PLOS One Bioinformatics (higher acceptance is likely)
    \item Briefings in Bioinformatics Oxford
    \item 
\end{itemize}
